Test-Time Adaptation for Combating Missing Modalities in Egocentric Videos

Understanding videos that contain multiple modalities is crucial, especially in egocentric videos, where combining various sensory inputs significantly improves tasks like action recognition and moment localization. However, real-world applications often face challenges with incomplete modalities due to privacy concerns, efficiency needs, or hardware issues. Current methods, while effective, often necessitate retraining the model entirely to handle missing modalities, making them computationally intensive, particularly with large training datasets. In this study, we propose a novel approach to address this issue at test time without requiring retraining. We frame the problem as a test-time adaptation task, where the model adjusts to the available unlabeled data at test time. Our method, MiDl~(Mutual information with self-Distillation), encourages the model to be insensitive to the specific modality source present during testing by minimizing the mutual information between the prediction and the available modality. Additionally, we incorporate self-distillation to maintain the model's original performance when both modalities are available. MiDl represents the first self-supervised, online solution for handling missing modalities exclusively at test time. Through experiments with various pretrained models and datasets, MiDl demonstrates substantial performance improvement without the need for retraining.

==> tables/ego4d_warmup.tex <==
\begin{table}[t]
    \caption{\textbf{Adaptation at Test-time with Ego4D warm-up.} We show another use cause of MiDL, in which the assumption is having access to out-of-domain unlabeled data to adapt before deployment. The results showcase MiDL's capabilities on leveraging unlabeled-out-of-domain data to combat missing modalities.}
    \centering
    \small
    \begin{tabular}{l|ccccc|ccccc}
         \toprule
         & \multicolumn{5}{c|}{Epic-Sounds (\%)}& \multicolumn{5}{c}{Epic-Kitchens (\%)} \\
         \multirow{-2}{*}{\diagbox{Model}{$1-p_{AV}$}}&0 & 25& 50& 75& 100 & 0 & 25& 50& 75& 100 \\
         \midrule
         % Unimodal & 41.4&41.4&41.4&41.4&41.4  &40.0&40.0&40.0&40.0 &40.0 \\
         Baseline & \textbf{55.1}&45.6&37.1&28.3& \textbf{19.5} &63.9& 55.5& 46.8& 37.9& 29.5 \\
         
         % \midrule
            +MiDl (ours) & 55.0 & \textbf{46.8} & \textbf{38.8} & 29.8 & 
            \textbf{19.5} & 63.7 & \textbf{58.4}& \textbf{52.4} & 46.4 & 29.5 \\
          $\,\,\,$ + Ego4D Warm-up& 55.0	&46.6	& 38.6	&\textbf{30.8}& 9.5 & 63.7&	\textbf{58.4}&	\textbf{52.4}&	\textbf{46.7}&	\textbf{37.8}\\
         \midrule \bottomrule
    \end{tabular}
    \label{tab:ego4d}
\end{table}





==> tables/mmt.tex <==
Waiting for numbers

==> tables/self_attention.tex <==
% \begin{table}[t]
%     \caption{Adaptation at Test-time on Epic Kitchen}
%     \centering
%     \begin{tabular}{l|cc|ccccc}
%          \toprule

%          {\diagbox{Model}{$1-p_{AV}$}}& $\mathcal L_\text{MI}$ & $\mathcal L_\text{KL}$ &0(\%) & 25(\%)& 50(\%)& 75(\%)& 100(\%)  \\
%          \midrule
%          Baseline & \xmark & \xmark & 45.3	&38.8&	32.7&	26.7&	20.5 \\
%          & \xmark & \cmark  & 45.3	&38.8&	32.7&	26.7&	20.5\\
%          & \cmark & \xmark  & \\
%          \midrule
%          MiDl (ours) & \cmark & \cmark & 45.5&	39.5&	33.8&	27.5&	20.5 \\
%          \midrule \bottomrule
%     \end{tabular}
%     \label{tab:components_of_midl}
% \end{table}



\begin{table}[t]
    \caption{\textbf{MiDL performance under a different architecture.} We showcase the effectiveness of MiDL when applied to a distinct baseline architecture characterized by multimodal self-attention. MiDL enhances performance across all missing rates, underscoring its robustness and adaptability to various underlying architectures.}
    \centering
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|ccccc}
         \toprule
         \multirow{2}{*}{\diagbox{Model}{$1-p_{AV}$}}& \multicolumn{5}{c}{Epic Sounds (\%)}\\
         &0&25&50&75&100\\
         \midrule
         % Unimodal & 46.5&	46.5&	46.5&	46.5&	46.5 \\
         Self-Attention Baseline & 45.3	&38.8&	32.7&	26.7&	20.5 \\
         % \midrule
         +Shot & 45.7&	38.7&	32.6&	26.4	&20.5 \\
         % Tent &      \\
         +ETA & 45.3&	37.9&	32.8&	26.7	&20.5 \\
         \midrule
         +MiDl (ours) & 45.5&	39.5&	33.8&	27.5&	20.5 \\
         +MiDl - LTA (ours) & 45.5	&\textbf{39.6}&	\textbf{34.5}&	\textbf{29.0}&	\textbf{23.2} \\
         \midrule \bottomrule
    \end{tabular}
    \label{tab:self_attention}
\end{table}
